Searching for polarization in signed graphs: a local spectral approach

Signed graphs have been used to model interactions in social net-works, which can be either positive (friendly) or negative (antagonistic). The model has been used to study polarization and other related phenomena in social networks, which can be harmful to the process of democratic deliberation in our society. An interesting and challenging task in this application domain is to detect polarized communities in signed graphs. A number of different methods have been proposed for this task. However, existing approaches aim at finding globally optimal solutions. Instead, in this paper we are interested in finding polarized communities that are related to a small set of seed nodes provided as input. Seed nodes may consist of two sets, which constitute the two sides of a polarized structure. In this paper we formulate the problem of finding local polarized communities in signed graphs as a locally-biased eigen-problem. By viewing the eigenvector associated with the smallest eigenvalue of the Laplacian matrix as the solution of a constrained optimization problem, we are able to incorporate the local information as an additional constraint. In addition, we show that the locally-biased vector can be used to find communities with approximation guarantee with respect to a local analogue of the Cheeger constant on signed graphs. By exploiting the sparsity in the input graph, an indicator vector for the polarized communities can be found in time linear to the graph size. Our experiments on real-world networks validate the proposed algorithm and demonstrate its usefulness in finding local structures in this semi-supervised manner.

==> acmart-master/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> acmart-master/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> compl_slackness.tex <==
\begin{claim}
  \label{claim:conditions}
  The following feasibility and complementary slackness conditions are sufficient for a primal-dual pair $\Xopt$, $(\alphaopt, \betaopt)$ to be an optimal solution.
  
  The feasibility conditions are:
  \begin{align}
    \label{eq:feas1} \dmat  \mprod \Xopt & = 1,  \\
    \dsds \mprod \Xopt & \ge \kappa, \nonumber \\
    \Xopt &\geneq 0 \nonumber \\
    \label{eq:feas2}\lap - \alphaopt \dmat - \betaopt \dsds & \geneq  0, \: and \\
    \betaopt & \ge 0 \nonumber
  \end{align}

  and complementary slackness conditions are:
  \begin{align}
    \label{eq:cs1} \betaopt (\dsds \mprod \Xopt  - \kappa) & = 0, \: and \\
    \label{eq:cs2} \Xopt \mprod (\lap - \alphaopt \dmat - \betaopt \dsds) &= 0
  \end{align}
\end{claim}

==> data/casestudy2.tex <==
v% This file was created by matplotlib2tikz v0.7.4.
\begin{tikzpicture}

\definecolor{color1}{rgb}{1,0,1}
\definecolor{color0}{rgb}{0,1,1}

\begin{axis}[
tick align=outside,
x grid style={white!69.01960784313725!black},
xmajorticks=false,
xmin=-1.10764592953362, xmax=0.957019870934199,
% xtick style={color=black},
y grid style={white!69.01960784313725!black},
ymajorticks=false,
ymin=-0.247603946792773, ymax=0.263008778699399,
% ytick style={color=black}
axis lines=none
]

\tikzset{%
  line style/.style={%
    line width=1.5pt
  }
}

\path [line style, draw=red, draw opacity=0.5, dash pattern=on 3.7pt off 1.6pt]
(axis cs:0.551295067517896,0.0484914477210859)
--(axis cs:-0.802507411277838,-0.0309067662217074);

\path [line style, draw=red, draw opacity=0.5, dash pattern=on 3.7pt off 1.6pt]
(axis cs:0.551295067517896,0.0484914477210859)
--(axis cs:-0.582973997592881,-0.083071238090259);

\path [line style, draw=red, draw opacity=0.5, dash pattern=on 3.7pt off 1.6pt]
(axis cs:0.551295067517896,0.0484914477210859)
--(axis cs:-0.732331457727241,-0.162848009799864);

\path [line style, draw=red, draw opacity=0.5, dash pattern=on 3.7pt off 1.6pt]
(axis cs:0.56463948963679,0.230652841327966)
--(axis cs:-0.872441696300246,-0.20314980696585);

\path [line style, draw=red, draw opacity=0.5, dash pattern=on 3.7pt off 1.6pt]
(axis cs:-0.802507411277838,-0.0309067662217074)
--(axis cs:0.651854197594556,0.0697209548204481);

\path [line style, draw=red, draw opacity=0.5, dash pattern=on 3.7pt off 1.6pt]
(axis cs:-0.802507411277838,-0.0309067662217074)
--(axis cs:0.856423309630576,0.141983446750479);

\path [line style, draw=red, draw opacity=0.5, dash pattern=on 3.7pt off 1.6pt]
(axis cs:-1,0.0447780574736638)
--(axis cs:0.651854197594556,0.0697209548204481);

\path [line style, draw=red, draw opacity=0.5, dash pattern=on 3.7pt off 1.6pt]
(axis cs:-1,0.0447780574736638)
--(axis cs:0.856423309630576,0.141983446750479);

\path [line style, draw=red, draw opacity=0.5, dash pattern=on 3.7pt off 1.6pt]
(axis cs:0.651854197594556,0.0697209548204481)
--(axis cs:-0.916233562124976,0.145747289398326);

\path [line style, draw=red, draw opacity=0.5, dash pattern=on 3.7pt off 1.6pt]
(axis cs:0.651854197594556,0.0697209548204481)
--(axis cs:-0.732331457727241,-0.162848009799864);

\path [line style, draw=red, draw opacity=0.5, dash pattern=on 3.7pt off 1.6pt]
(axis cs:0.534691591458832,-0.0669272098346593)
--(axis cs:-0.732331457727241,-0.162848009799864);

\path [line style, draw=red, draw opacity=0.5, dash pattern=on 3.7pt off 1.6pt]
(axis cs:0.856423309630576,0.141983446750479)
--(axis cs:-0.916233562124976,0.145747289398326);

\path [line style, draw=red, draw opacity=0.5, dash pattern=on 3.7pt off 1.6pt]
(axis cs:0.614572144064517,-0.0955759510872597)
--(axis cs:-0.732331457727241,-0.162848009799864);

\path [line style, draw=red, draw opacity=0.5, dash pattern=on 3.7pt off 1.6pt]
(axis cs:0.696672346105145,-0.0718444753221874)
--(axis cs:-0.732331457727241,-0.162848009799864);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:0.551295067517896,0.0484914477210859)
--(axis cs:0.56463948963679,0.230652841327966);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:0.551295067517896,0.0484914477210859)
--(axis cs:0.651854197594556,0.0697209548204481);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:0.551295067517896,0.0484914477210859)
--(axis cs:0.43633997901487,0.0329494198298172);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:0.551295067517896,0.0484914477210859)
--(axis cs:0.534691591458832,-0.0669272098346593);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:0.551295067517896,0.0484914477210859)
--(axis cs:0.614572144064517,-0.0955759510872597);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:0.551295067517896,0.0484914477210859)
--(axis cs:0.696672346105145,-0.0718444753221874);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:0.56463948963679,0.230652841327966)
--(axis cs:0.651854197594556,0.0697209548204481);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:-0.802507411277838,-0.0309067662217074)
--(axis cs:-1,0.0447780574736638);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:-0.802507411277838,-0.0309067662217074)
--(axis cs:-0.916233562124976,0.145747289398326);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:-0.802507411277838,-0.0309067662217074)
--(axis cs:-0.872441696300246,-0.20314980696585);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:-0.802507411277838,-0.0309067662217074)
--(axis cs:-0.582973997592881,-0.083071238090259);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:-0.802507411277838,-0.0309067662217074)
--(axis cs:-0.732331457727241,-0.162848009799864);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:-1,0.0447780574736638)
--(axis cs:-0.916233562124976,0.145747289398326);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:0.651854197594556,0.0697209548204481)
--(axis cs:0.43633997901487,0.0329494198298172);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:0.651854197594556,0.0697209548204481)
--(axis cs:0.534691591458832,-0.0669272098346593);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:0.651854197594556,0.0697209548204481)
--(axis cs:0.856423309630576,0.141983446750479);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:0.651854197594556,0.0697209548204481)
--(axis cs:0.614572144064517,-0.0955759510872597);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:0.651854197594556,0.0697209548204481)
--(axis cs:0.696672346105145,-0.0718444753221874);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:0.43633997901487,0.0329494198298172)
--(axis cs:0.534691591458832,-0.0669272098346593);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:0.534691591458832,-0.0669272098346593)
--(axis cs:0.614572144064517,-0.0955759510872597);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:0.534691591458832,-0.0669272098346593)
--(axis cs:0.696672346105145,-0.0718444753221874);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:0.614572144064517,-0.0955759510872597)
--(axis cs:0.696672346105145,-0.0718444753221874);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:-0.872441696300246,-0.20314980696585)
--(axis cs:-0.732331457727241,-0.162848009799864);

\path [line style, draw=blue, draw opacity=0.5]
(axis cs:-0.582973997592881,-0.083071238090259)
--(axis cs:-0.732331457727241,-0.162848009799864);

% \addplot [only marks, draw=color0, fill=color0, opacity=0.5, colormap/viridis]
\addplot [only marks, draw=color0, fill=color0, opacity=0.5]
table{%
x                      y
-0.916233562124976 0.145747289398326
-0.802507411277838 -0.0309067662217074
-1 0.0447780574736638
-0.582973997592881 -0.083071238090259
-0.732331457727241 -0.162848009799864
-0.872441696300246 -0.20314980696585
};
% \addplot [only marks, draw=color1, fill=color1, opacity=0.5, colormap/viridis]
\addplot [only marks, draw=color1, fill=color1, opacity=0.5]
table{%
x                      y
0.696672346105145 -0.0718444753221874
0.614572144064517 -0.0955759510872597
0.534691591458832 -0.0669272098346593
0.651854197594556 0.0697209548204481
0.551295067517896 0.0484914477210859
0.856423309630576 0.141983446750479
0.43633997901487 0.0329494198298172
0.56463948963679 0.230652841327966
};
% \addplot [only marks, draw=green!50.19607843137255!black, fill=green!50.19607843137255!black, colormap/viridis]
% table{%
% x                      y
% -0.916233562124976 0.145747289398326
% -0.802507411277838 -0.0309067662217074
% };
% \addplot [draw=none, draw=blue, fill=blue, colormap/viridis]
% table{%
% x                      y
% -0.5 -0.5
% 0.5 -0.5
% 0.5 0.5
% -0.5 0.5
% -0.5 -0.5
% };
\addplot [ultra thick, blue]
table {%
-0.7 0.24
-0.35 0.24
};
\addplot [ultra thick, red, dashed]
table {%
-0.7 0.19
-0.35 0.19
};
\node at (axis cs:-0.902507411277838,0.0159067662217074)[
  scale=1.3,
  text=black,
  rotate=0.0
]{female};
\node at (axis cs:-1.01623356212498,0.160747289398326)[
  scale=1.3,
  text=black,
  rotate=0.0
]{fair};
\node at (axis cs:-0.682973997592881,-0.068071238090259)[
  scale=1.3,
  text=black,
  rotate=0.0
]{lady};
\node at (axis cs:-0.832331457727241,-0.127848009799864)[
  scale=1.3,
  text=black,
  rotate=0.0
]{woman};
\node at (axis cs:0.44463948963679,0.245652841327966)[
  scale=1.3,
  text=black,
  rotate=0.0
]{son};
\node at (axis cs:0.551854197594556,0.1057209548204481)[
  scale=1.3,
  text=black,
  rotate=0.0
]{male};
\node at (axis cs:0.33633997901487,-0.0079494198298172)[
  scale=1.3,
  text=black,
  rotate=0.0
]{brother};
\node at (axis cs:0.434691591458832,-0.0519272098346593)[
  scale=1.3,
  text=black,
  rotate=0.0
]{guy};
\node at (axis cs:0.606423309630576,0.176983446750479)[
  scale=1.3,
  text=black,
  rotate=0.0
]{masculine};
\node at (axis cs:-0.3,0.23)[
  scale=1.4,
  anchor=base west,
  text=black,
  rotate=0.0
]{$\posedges$};
\node at (axis cs:-0.3,0.18)[
  scale=1.4,
  anchor=base west,
  text=black,
  rotate=0.0
]{$\negedges$};
\end{axis}

\end{tikzpicture}

==> syn_exp_figs_old.tex <==
\begin{figure*}[!h]
  \centering
  \newcommand{\addfigure}[1]{\includegraphics[width=0.31\linewidth]{synthetic_experiment/#1.pdf}}  
  \begin{tabular}{ccc}
    Effect of node noise & Effect of edge noise & Effect of seed size \\
    \addfigure{{effect_of_outlier_solution_size}} & \addfigure{{effect_of_eta_solution_size}} & \addfigure{{effect_of_seed_solution_size}} \\
    (a) & (b) & (c) \\
    \addfigure{{effect_of_outlier_beta_ratio}} & \addfigure{{effect_of_eta_beta_ratio}} & \addfigure{{effect_of_seed_beta_ratio}} \\
    (d)  & (e)  & (f) \\
    \addfigure{{effect_of_outlier_ap}} & \addfigure{{effect_of_eta_ap}} & \addfigure{{effect_of_seed_ap}} \\
    (g)  & (h)  & (i)                     
  \end{tabular}
  \caption{
    % \inote{Fix the caption because new row of sub figures}
    Performance of different metrics on synthetic graphs.
    \textbf{Top}: solution volume, $\vol(\Sone \cup \Stwo)$.
    \textbf{middle}: \sbr ratio, $\sbr(\Sone, \Stwo) / \sbr(\Sonetrue, \Stwotrue)$.
    and \textbf{bottom}: average precision (\ap);
    % and \textbf{bottom}: solution size, $\abs{\Sone \cup \Stwo}$.
    We vary 3 parameters:
    (i) number of outlier nodes $\outliercount$;
    (ii) edge noise parameter $\noise$;
    (iii) seed size $\seedcount$ for $\Sonetrue$ and $\Stwotrue$.
    Results are shown for 3 values of the parameter $\kappa$.
    % For each configuration, the result is obtained by averaging over 10 random graphs and 32 random seeds.
    In figure (e), we use a red solid line at $y=1$  to differentiate two cases of $\sbr$ ratio.
    Error bars at 0.95 confidence interval is drawn in the form of shaded area. 
    % In figure (g)-(i), solid red lines are drawn horizontally at $\abs{\Sonetrue \cup \Stwotrue}$.
  }
  \label{fig:syn}
\end{figure*}

